Debias Coarsely, Sample Conditionally: Statistical Downscaling through Optimal Transport and Probabilistic Diffusion Models

We introduce a two-stage probabilistic framework for statistical downscaling using unpaired data. Statistical downscaling seeks a probabilistic map to transform low-resolution data from a biased coarse-grained numerical scheme to high-resolution data that is consistent with a high-fidelity scheme. Our framework tackles the problem by composing two transformations: (i) a debiasing step via an optimal transport map, and (ii) an upsampling step achieved by a probabilistic diffusion model with a posteriori conditional sampling. This approach characterizes a conditional distribution without needing paired data, and faithfully recovers relevant physical statistics from biased samples. We demonstrate the utility of the proposed approach on one- and two-dimensional fluid flow problems, which are representative of the core difficulties present in numerical simulations of weather and climate. Our method produces realistic high-resolution outputs from low-resolution inputs, by upsampling resolutions of 8x and 16x. Moreover, our procedure correctly matches the statistics of physical quantities, even when the low-frequency content of the inputs and outputs do not match, a crucial but difficult-to-satisfy assumption needed by current state-of-the-art alternatives. Code for this work is available at: https://github.com/google-research/swirl-dynamics/tree/main/swirl_dynamics/projects/probabilistic_diffusion.

==> intro-old.tex <==
\section{Introduction}
\label{sIntro}

Advances in computational and modeling techniques have fueled the development of global circulation models (GCMs), which have become the backbone of weather forecasting and climate modeling. The computational complexity of GCMs grows rapidly with resolution\footnote{For instance, doubling the resolution, i.e., the number of grid points in each of three dimensions, requires making the time step shorter to satisfy the CFL condition, which results in a cost scaling to the fourth power.}
%\todo{This should be third power, right? if you model the atmosphere in 3d you have 3 powers, and then you need to account for the CFL condition for the time discretization.}
, which severally limits the resolution of long-running climate simulations. As a result, predictions are often made with coarse low-resolution models and are confronted with two issues: \textit{i)} they contain inherent bias from a lack of representation of small-scale dynamics \cite{Christensen2008,Zelinka2020}, and \textit{ii)} they lack the granularity necessary to be of practical use for regional or local climate impacts studies \cite{Grotch1991:GCMforclimate}, such as the prediction or risk assessment of extreme flooding \cite{Gutmann2014:statistical_downscaling_water_resources,Hwang2014:Statistical_Downscaling_precipitations}, heat waves, or wildfires \cite{Abatzoglou2012:downscaling_wildfire}.

In this context, statistical downscaling \cite{Wilby_1998:downscaling,Wilby:2006} learns a map from low- to high-resolution data by leveraging statistical properties of the data stemming from a high-resolution model. At its core, the objectives of statistical downscaling are two-fold: to provide high-resolution features and to correct biases induced by the low-resolution model. 
% \todo{perhaps remove this? it is true but it if kind of off message.}In addition, it is also important to measure the uncertainty in this mapping, due to the ill-posed nature of the inverse problem.

At the algorithmic level, the core difficulty of statistical downscaling is the lack of \textit{aligned data}: there is no natural pairing of samples from the low-resolution model (such as climate models \cite{Danabasoglu2020:cesm}) with samples from higher-resolution ones (such as weather models that assimilate observations \cite{hersbach2020era5}).
% In practice, we do not have high-resolution data of how the earth would look like in the future, and the models output a climate that we have not seen.
Even in simplified cases of idealized fluids simulations, it is hard to align the datasets, due to the chaotic behavior of the models: two simulations with very close initial conditions will diverge rapidly.
% and their own biases, induced by modelling choices and the different resolution.


Several recent studies in climate sciences have focused on showcasing the advantages of machine-learning (ML) techniques for tackling this problem \cite{pan2021learning,harris2022generative,price2022increasing,hammoud2022cdanet} when compared to traditional approaches \cite{BurgerDownscaling:2012}. Despite the encouraging results, most of these studies rely on synthetically generated paired datasets of high- and low-resolution measurements to learn bias-correction models via supervised learning approaches (e.g., conditional GANs). Such paired datasets are often generated intrusively by manipulating model outputs, e.g., by using low-resolution data as boundary conditions in high-resolution models \cite{dixon2016evaluating,Huang2020:forced_paired_data}, or by nudging the low-resolution model towards high-resolution trajectories \cite{charalampopoulos2023statistics}. Unfortunately, requiring paired data for training severely limits the potential applicability of such methodologies to downstream tasks. 

% In climate sciences, downscaling low-resolution climate simulations leveraging machine-learning tools have been applied to various forecasts of maximum temperature, and precipitation~\cite{pan2021learning,harris2022generative,price2022increasing,hammoud2022cdanet}; see \cite{BurgerDownscaling:2012} for a review of traditional techniques. Unfortunately, most of these studies rely on synthetically generated paired datasets of high- and low-resolution measurements and they rely on supervised learning (e.g., conditional GANs) to learn bias-correction models. Such paired datasets are often generated intrusively by manipulating model outputs, e.g., by using low-resolution data as boundary conditions in high-resolution models \cite{dixon2016evaluating,Huang2020:forced_paired_data}, or by nudging the low-resolution model towards high-resolution trajectories \cite{charalampopoulos2023statistics}. 



% In fact, several machine learning methodologies, such as GANs and VAEs, could, in theory, be easily repurposed to the super-resolution task provided that aligned data is available.

%namely: %\footnote{Perhaps we want a more mathematical description.}

% \leo{explain how we simplify the problem, while }
% In this paper, we present a novel and simple framework for probabilistic downscaling problem.  

% % \fs{Explain well the difference between these two axes and why climate model has to be low-resolution and low-fidelity}
% To use our framework to downscale coarse simulation of chaotic systems in one and two dimension. We assume that we have data coming from a high-resolution, high-fidelity model, which serves as ground truth.%, which could be the output of a weather model such as ERA5. 
% We also assume that we have a low-resolution, low-fidelity model, which can be run efficiently.
% % \fs{This is a risky to write the paper. Need better transition even if we focus on PoC}
% We point out that our examples captures some of the core multi-scale behavior of weather/climate data. 

% To use our framework to downscale fluids simulations. We assume that we have data coming from a high-resolution, high-fidelity model, which serves as ground truth, which could be the output of a weather model such as ERA5. We also assume that we have a \fs{Explain well the difference between these two axes and why climate model has to be low-resolution and low-fidelity}low-resolution, low-fidelity model, which emulates climate models. \fs{This is a risky to write the paper. Need better transition even if we focus on PoC}Instead of using weather data, we use one- and two-dimensional chaotic systems that captures some of the core multi-scale behavior of weather data. 

% \begin{figure}[h]
% \centering
% \vspace{-0.4cm}
% \includegraphics[height=3cm, trim={0.1cm 13cm 15cm 0cm}, clip]{Extrapolation_drawing.pdf}
% \hspace{0.3cm}
% \includegraphics[height=3cm, trim={0.1cm 4cm 8cm 0cm}, clip]{diagram_method.pdf}
% \vspace{-0.5cm}
% \caption{(Left): Super-resolution as frequency extrapolation in the Fourier domain. The diffusion model extrapolates low-frequency content to higher-frequencies (dashed blue). The debiasing map corrects the biased low-frequency content (solid red). (Right): Diagram of the proposed framework where $C',C$ are unknown and known downsampling maps, respectively, and $T$ is the debiasing map.}
% \label{fig:framework_diagram}
% \end{figure}

\begin{figure}[!ht]
  \vspace{-1cm}
  \centering
  {\setlength\tabcolsep{1.5pt}
      \begin{tabular}{M{.4\linewidth}M{.55\linewidth}}
        \includegraphics[height=4.5cm, trim={0.1cm 13cm 15cm 0cm}, clip]{Extrapolation_drawing.pdf}  \vspace{-25pt} &
        \hspace{2cm} \includegraphics[height=4.5cm, trim={0.1cm 4cm 8cm 0cm}, clip]{diagram_method.pdf} \vspace{-25pt} \\
        \hspace{30pt} (a)  & \hspace{40pt} (b) 
      \end{tabular}
  }
  \caption{(a) Super-resolution as frequency extrapolation in the Fourier domain. The diffusion model extrapolates low-frequency content to higher-frequencies (dashed blue). The debiasing map corrects the biased low-frequency content (solid red). (b) Diagram of the proposed framework where $C',C$ are unknown and known downsampling maps, respectively, and $T$ is the debiasing map.}
  \vspace{-.4cm}
  \label{fig:framework_diagram}
\end{figure}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[height=3cm, trim={0.1cm 13cm 15cm 0cm}, clip]{Extrapolation_drawing.pdf}
%          \caption{$y=x$}
%          \label{fig:extrapolation}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[height=3cm, trim={0.1cm 4cm 8cm 0cm}, clip]{diagram_method.pdf}
%          \caption{$y=3\sin x$}
%          \label{fig:diagram_network}
%      \end{subfigure}
%     \caption{(a): Super-resolution as frequency extrapolation in the Fourier domain. The diffusion model extrapolates low-frequency content to higher-frequencies (dashed blue). The debiasing map corrects the biased low-frequency content (solid red). (b): Diagram of the proposed framework where $C',C$ are unknown and known downsampling maps, respectively, and $T$ is the debiasing map.}
%     \label{fig:framework_diagram}
% \end{figure}

% We seek to tackcl this issue by proposing a new \text{probabilistic} formulation for the downscaling problem that handles \textit{unpaired data} directly, 
We propose a new \text{probabilistic} formulation for the downscaling problem that handles \textit{unpaired data} directly, 
while leveraging recent advances in generative models and domain adaption, in particular probabilistic diffusion models \cite{song2020score} and optimal transport \cite{cuturi2013sinkhorn}. This new formulation composes two procedures: a debiasing step followed by a super-resolution one. The debiasing step is performed by an optimal transport map learned using unpaired data, while the super-resolution step is performed by using a probabilistic diffusion model for conditional sampling. % with conditional sampling, without paired data. 
%We also introduce an intermediate space between these two steps from downsampling high-resolution data to match the dimensions of the low-resolution data; see Figure~\ref{fig:framework_diagram} (left).

% A core advantage of probabilistic models for super-resolution is their ability to generate samples that are consistent with the low-resolution snapshots, and thus provide a measure of the uncertainty of the high-resolution predictions, which is of key for downstream applications. %On the other hand, the debiasing map corrects the biased Fourier spectrum of an input to render it admissible with respect to the target resolution.
% However, this requires the low-resolution data to already contain the correct statistical information, for which debiasing is key. In fact, super-resolution can be recast as frequency extrapolation \cite{Candes2016:Superresolution}, in which the model reconstructs high-frequency content (i.e., the blue dashed line in Fig.~\ref{fig:framework_diagram} (left)) while restricting low-frequency content (i.e., the solid blue line in Fig.~\ref{fig:framework_diagram} (left)) to match those from the low-resolution input. However, the restriction of the target high-resolution data %has its own distribution in Fourier space , whose restriction 
% may not match the distribution of the low-resolution data in Fourier space~\cite{kolmogorov1962refinement} (i.e., the solid red line in Fig.~\ref{fig:framework_diagram} (left)). debiasing, therefore corrects the Fourier spectrum of the low-resolution input to render it admissible for the target distribution (i.e., moving solid red to solid blue lines in Fig.~\ref{fig:framework_diagram} (left)).

\textbf{Intuition.} Our framework relies on two key properties. First, we leverage the ability of probabilistic models for super-resolution to \emph{generate samples} that are consistent with the low-resolution snapshots~\cite{Li2022:SRDiff}, to provide a measure of the uncertainty of the high-resolution predictions. Unfortunately, this implies that %incorrect statistics, or biases, of 
biases of the low-resolution snapshots will pollute the end results. Second, we leverage the ability of optimal transport techniques~\cite{villani2009optimal} to \emph{preserve the marginal distributions},  
to correct the %statistics
biases of the low-resolution snapshots, thereby resulting in high-resolution snapshots with the correct statistics.
%and which results in high-resolution snapshots with the correct statistics. 

The intuition of our framework is depicted in Fig.~\ref{fig:framework_diagram}(a). Super-resolution can be recast as frequency extrapolation \cite{Candes2016:Superresolution}, in which the model reconstructs high-frequency content 
while matching the low-frequency content 
of a low-resolution input. However, the restriction of the target high-resolution data 
may not match the distribution of the low-resolution data in Fourier space~\cite{kolmogorov1962refinement}. 
Debiasing, therefore corrects the Fourier spectrum of the low-resolution input to render it admissible for the target distribution (moving solid red to solid blue lines with the  dashed blue extrapolation in Fig.~\ref{fig:framework_diagram}). \todo{Leo: I moved this one here from the paragraph below}This allows us to bypass the crucial but difficult-to-satisfy requirement that the low-frequency statistics of the low- and high-resolution datasets need to match. 

We showcase the performance of this framework on idealized fluids problems that preserve the core difficulty of atmospherics flows. We show that our framework is able to generate realistic snapshots that are faithful to the physical statistics.
% and it does not require the low-frequency statistics of the low- and high-resolution datasets to match, which is a crucial but difficult-to-satisfy assumption.



% One of the main limitations of deterministic climate downscaling modeling is that its only provides one particular answer, even though it is highly plausible that many snapshots in the target distribution can provide a similar downsampled field. This one solution doesn't not provide any uncertainty measurements, and it does not account for possible errors in the measurement. 
% \paragraph{Why debiasing?}
% (TODO: rewrite this to it is clearer, also add a picture).
% One can see super-resolution in Fourier domain as frequency extrapolation. Basically, we provide a certain constraint on the frequency content at low-frequency and the model then reconstructs the higher-frequency content. Mathametically this process can be achieved when the extrapolation is mild and the underlying signal has some structure, such as sparsity in Fourier domain, and several optimization based algorithm have been proposed (cite Candes and Fernandez-Grande). Neural networks, on the other hand, are able to generate higher-resolution images without these resctrictions. In this case, then it is important that the to-be-superresolved image has a Fourier spectrum admissible for the distributions in the target space. 
% \paragraph{Advantages}
% The main advantages of the proposed method are summarized below: \todo{What do you think of making these into contributions? Should these advantages come after the paragraphs on why probabilistic models and debiasing?}
% \begin{itemize}
%     \item we provide a probabilistic approach, which can be also used to measure the likely hood of a certain configuration, under certain conditions.
%     \item There is no need to create paired data.
%     \item we can easily iterate, and even optimize with respect to either the transport map of the linear-downsamplign map. 
%     \item The unconditional model for the high-resolution high-fidelity marginal needs to be trained only once, which is often the most expensive step during training. 
% \end{itemize}

==> rebuttal.tex <==
\section*{Additional Figures}

\setcounter{figure}{0}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/rebuttal/sample_comparison_8x_and_16x_unlabeled_rebuttal.pdf}
{\setlength\tabcolsep{0.4pt}
\begin{tabular}{M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}M{.11\linewidth}}
     (a) & (b) & (c) & (d) & (e) & (f) & (g)  & (h) & (i)
\end{tabular}
}
\caption{\textbf{[Figure 3 updated with additional baselines]} Example showing the vorticity field of samples debiased and super-resolved using different techniques at $8\times$ (top row) and $16\times$ (bottom row) downscaling factors. From left to right: (a) LR snapshot produced by the low-fidelity solver (input $\bar{y}$ of Alg. \ref{alg:inference}), (b) OT-corrected snapshot ($\bar{y}'$ in line $1$ of Alg. \ref{alg:inference}), \textbf{(c) BCSD}, (d) downscaled snapshot with cycle-GAN directly from LR snapshot, \textbf{(e) ClimAlign}, (f) cubic interpolation of the OT-corrected snapshot, (g) deterministic upsample of the OT-corrected snapshot, (h) diffusion sample conditioned on the OT-corrected snapshot (output $\bar{x}$ in Alg.~\ref{alg:inference}), and (i) two true HR samples in the training data with the closest Euclidean distance to the OT-corrected generated sample. The $16\times$ source is the same as the $8\times$ source but further downsampled by a factor of two. OT maps are computed independently between resolutions.}
% \caption{Updated Figure 3}
\label{fig:rebuttal_samples}
\end{figure}

\begin{figure}[h]
  \centering
  {\setlength\tabcolsep{0.5pt} {\renewcommand{\arraystretch}{0.5}
      \begin{tabular}{M{.45\linewidth}M{.45\linewidth}}
        
        \hspace{-3pt}\includegraphics[width=\linewidth]{figures/rebuttal/ns_spec_logratio_compare_8xds_rebuttal.pdf} & 
        \hspace{-3pt}\includegraphics[width=\linewidth]{figures/rebuttal/ns_spec_logratio_compare_16xds_rebuttal.pdf} \\
        (a) NS $8\times$, log energy ratios & \quad (b) NS $16\times$, log energy ratios \\
      \end{tabular}
  }}
  \caption{\textbf{[Updated energy ratio plots 2(c) and 4(c) with additional baselines]} mode-wise log energy ratios with respect to the true samples (\eqref{eq:MELR} without weighted sum) at (a) $8\times$ and (b) $16\times$ downscaling for NS.}
  \label{fig:rebuttal_energy_plots}
\end{figure}

